Formal Verification of Spacecraft Control Programs Using a Metalanguage for State Transformers

Verification of functional correctness of control programs is an essential task for the development of space electronics; it is difficult and time-consuming and typically outweighs design and programming tasks in terms of development hours. We present a verification approach designed to help spacecraft engineers reduce the effort required for formal verification of low-level control programs executed on custom hardware. The approach uses a metalanguage to describe the semantics of a program as a state transformer, which can be compiled to multiple targets for testing, formal verification, and code generation. The metalanguage itself is embedded in a strongly-typed host language (Haskell), providing a way to prove program properties at the type level, which can shorten the feedback loop and further increase the productivity of engineers. The verification approach is demonstrated on an industrial case study. We present REDFIN, a processing core used in space missions, and its formal semantics expressed using the proposed metalanguage, followed by a detailed example of verification of a simple control program.

==> tex/instructions.tex <==
The instruction set of REDFIN comprises~(\textbf{TODO:} a lot) instructions.
I doubt there is any rational reason in describing every instruction in the paper.
It would be nice to cite the REDFIN ISA manual, but it probably isn't publicly
availible.

Let's just have the IAM instructions description as a stub for the moment.

\begin{longtable}{l|p{9cm}}
\texttt{load r memaddr}     & Load a value from a memory location to a register.\\
\texttt{loadmi r memaddr}   & Load a value from the memory location to the register using
an indirect memory access mode\footnote{Loading the value from a memory location and using it as
a memory address argument for the~\texttt{load} instruction.}.\\
\texttt{set      r byte   } & Load an 8-bit immediate argument to a register.\\
\texttt{store    r memaddr} & Store a value from a register to a memory location.\\
\texttt{add      r memaddr} & Add a value placed in a memory location to a value contained in a register.\\
\texttt{jump     byte     } & Perform an unconditional jump modifying the machine
instruction counter by a given offset.\\
\texttt{jumpz    byte     } & Performs a conditional jump if the zero flag is set.\\
\texttt{halt              } & Stop the execution setting the halt flag.
\end{longtable}

We encode the instructions in Haskell using the following data type:

\begin{figure}[H]
\begin{minted}{haskell}
data Instruction = Load     Register MemoryAddress
                 | LoadMI   Register MemoryAddress
                 | Set      Register Byte
                 | Store    Register MemoryAddress
                 | Add      Register MemoryAddress
                 | Jump     Byte
                 | JumpZero Byte
                 | Halt
\end{minted}
\caption{Haskell data type representing IAM instructions.}
\label{Instruction}
\end{figure}

The~\mintinline{haskell}{JumpZero} and~\mintinline{haskell}{Halt} instructions'
operation depend on zero and halting flags values. Consider the definition
of~\mintinline{haskell}{Flags} data type:

\begin{figure}[H]
\begin{minted}{haskell}
data Flag = Zero
          | Halted
\end{minted}
\caption{Haskell data type representing IAM flags.}
\label{Flags}
\end{figure}

Let us clarify the other data types involved. The current implementation of the
formal verification framework is build on top of Haskell SBV (SMT Based Verification)
library~\cite{SBV}. SBV provides a DSL for defining properties to be automatically
checked by a SAT/SMT solver, and allows us to symbolically execute IAM programs.
The~\mintinline{haskell}{Register},~\mintinline{haskell}{MemoryAddress}
and~\mintinline{haskell}{Byte} types are internally represented as symbolic
SBV words of appropriate length.

Later in this report we will implement an interpreter for the IAM assembly language,
thus defining an operational semantics for the syntax provided.


==> tex/semantics.tex <==
\section{Instruction semantics}
\label{sec:Semantics}

In this section we define the meaning IAM instructions as a \emph{state
transformer}, i.e. a function from the state space to itself.

\begin{figure}[H]
\centering
$T = \{s_1 \rightarrow s_2 : s_1 \in S, s_2 \in S\}$
\label{}
\caption{A set of all machine state transformers.}
\end{figure}

Every instruction transforms the machine state in its own
way, thus we may define the instructions semantics as a mapping from instructions
to state transformers.

\begin{figure}[H]
\centering
$ \textrm{execute}:I \rightarrow T$
\label{}
\caption{Instruction interpreter.}
\end{figure}

Here $I$ is a finite set represented in Haskell as
the~\mintinline{haskell}{Instruction} data type.

The state transition representation is the core concept of the developed
Haskell framework. The Haskell's concept of~\emph{state monad} provides a way to
emulate a mutable state behaviour in a purely functional programming language
without explicit state threading. Consider the~\mintinline{haskell}{Machine} type being
essentially a parametrised state-transition builder:

\begin{figure}[H]
\begin{minted}{haskell}
newtype Machine a = Machine {runMachine :: State MachineState a}
\end{minted}
\caption{The IAM state transformer.}
\end{figure}

Every function with its return type market as~\mintinline{haskell}{Machine a} is a computation
yielding a value of type~\mintinline{haskell}{a} and possibly altering the state of the machine.

We define the semantics by implementing an interpreter
function~\mintinline{haskell}{execute} that considers every data constructor of
the~\mintinline{haskell}{Instruction} type and builds a computation in the
~\mintinline{haskell}{Machine} monad --- a transformer of IAM state. This function
is the heart of the simulation and formal verification framework.

\begin{figure}[H]
\begin{minted}{haskell}
execute :: Instruction -> Machine ()
execute (Halt                ) = executeHalt
execute (Load     rX dmemaddr) = executeLoad     rX dmemaddr
execute (LoadMI   rX dmemaddr) = executeLoadMI   rX dmemaddr
execute (Set      rX simm    ) = executeSet      rX simm
execute (Store    rX dmemaddr) = executeStore    rX dmemaddr
execute (Add      rX dmemaddr) = executeAdd      rX dmemaddr
execute (Jump     simm       ) = executeJump     simm
execute (JumpZero simm       ) = executeJumpZero simm
\end{minted}
\caption{An interpreter of IAM instruction set.}
\label{execute}
\end{figure}

Let us now consider the semantics of some of instructions.

The simplest state transformation is halting. If the interpreter sees the halt instruction, it
sets the~\mintinline{haskell}{Halted} flag preventing the following execution.
The~\mintinline{haskell}{writeFlag} does the actual machine state modification,
advancing the clock by one tick (using the~\mintinline{haskell}{delay} function)
and setting the flag.

\begin{figure}[H]
\begin{minted}{haskell}
executeHalt :: Machine ()
executeHalt = writeFlag Halted true

writeFlag :: Flag -> SBool -> Machine ()
writeFlag flag value = do
    delay 1
    modify $ \state ->
        state { flags = writeArray (flags state)
                                   (flagId flag)
                                   value }
\end{minted}
\caption{Semantics of the~\mintinline{haskell}{Halt} instruction.}
\label{haltSemantics}
\end{figure}

As a more involved example, let us define the semantics of the addition instruction.
It operates with a register containing a first term and a memory location referring
to the second one. The~\mintinline{haskell}{executeAdd} essentially retrieves the terms,
adds them, places the result to the register, and sets the \mintinline{haskell}{Zero}
flag if the result is zero.

\begin{figure}[H]
\begin{minted}{haskell}
executeAdd :: Register -> MemoryAddress -> Machine ()
executeAdd rX dmemaddr = do
    x <- readRegister rX
    y <- readMemory dmemaddr
    let z = x + y
    writeFlag Zero (z .== 0)
    writeRegister rX z
\end{minted}
\caption{Semantics of the~\mintinline{haskell}{Add} instruction.}
\label{addSemantics}
\end{figure}

Here,~\mintinline{haskell}{readRegister} and~\mintinline{haskell}{readMemory}
are functions dedicated to query the states of register bank and memory.
They are implemented in terms of SBV's array accessors:

\begin{figure}[H]
\begin{minted}{haskell}
readRegister :: Register -> Machine Value
readRegister register = do
    currentState <- get
    delay 1
    pure $ readArray (registers currentState) register

readMemory :: MemoryAddress -> Machine Value
readMemory address = do
    currentState <- get
    delay 2
    pure $ readArray (memory currentState) address
\end{minted}
\caption{Register bank and memory accessors.}
\label{readRegMem}
\end{figure}

Both functions retrieve the current state of the machine, advance the clock by
a predefined amount of cycles, and query the machine state for a desired value.

An interesting note to make here is that in the implementation of these functions
we are using Haskell as a~\emph{metalanguage}. We are operating the machine as
a puppet master, using the external meta-notions of addition, comparison and let-binding.
From the machine's point of view, we have an unlimited memory and act instantly,
which gives us an unlimited modeling power. Later in this section we'll see how
hard it is to achieve such a power using only IAM's internal entities.

As the most sophisticated example we give here, consider the semantics of the
\mintinline{haskell}{JumpZero} instruction. It uses SBV's symbolic conditional
operation~\mintinline{haskell}{ite} to test if the~\mintinline{haskell}{Zero} flag
is set, and, if so, modifies the machine's instruction counter by a provided offset.

\begin{figure}[H]
\begin{minted}{haskell}
executeJumpZero :: Byte -> Machine ()
executeJumpZero offset = do
    zeroIsSet <- readFlag Zero
    ic <- instructionCounter <$> get
    let ic' = ite zeroIsSet (ic + fromByte offset) ic
    modify $ \currentState ->
        currentState {instructionCounter = ic'}
\end{minted}
\caption{Semantics of the~\mintinline{haskell}{JumpZero} instruction.}
\label{jumpZeroSemantics}
\end{figure}

The semantics of the conditional jump instruction turns out to be one of the
most sensible parts of a verification framework that relies on symbolical execution.
It is vital to bear in mind the notion of~\emph{symbolic termination}. In our special
case the situation starts to get difficult if the instruction counter value becomes
purely symbolic, i.e. the program termination starts to depend on a symbolic value.
There are ways to control symbolic termination, but current state of implementation of
the verification framework is fragile and relies on the user to prevent the dangerous
situations from happening. Currently, the verification framework uses an external
counter of state transitions that guaranties termination.

The implementations of these three instruction interpreters cover all the interesting
features of the framework's implementation. Please consult to the framework
repository~\cite{IAMGithub} for the full source code.
